Penn-Helsinki Parsed Corpus of Early Modern English: First Parsing Results and Analysis

We present the first parsing results on the Penn-Helsinki Parsed Corpus of Early Modern English (PPCEME), a 1.9 million word treebank that is an important resource for research in syntactic change. We describe key features of PPCEME that make it challenging for parsing, including a larger and more varied set of function tags than in the Penn Treebank. We present results for this corpus using a modified version of the Berkeley Neural Parser and the approach to function tag recovery of Gabbard et al (2006). Despite its simplicity, this approach works surprisingly well, suggesting it is possible to recover the original structure with sufficient accuracy to support linguistic applications (e.g., searching for syntactic structures of interest). However, for a subset of function tags (e.g., the tag indicating direct speech), additional work is needed, and we discuss some further limits of this approach. The resulting parser will be used to parse Early English Books Online, a 1.1 billion word corpus whose utility for the study of syntactic change will be greatly increased with the addition of accurate parse trees.

==> previouswork.tex <==
\section{Previous Work}
\label{sec:previous}


The \ppceme is one of several corpora designed for historical linguistics research  that share annotation styles and design decisions.  Others include the
second edition of the Penn-Helsinki Parsed Corpus of Middle English \citep{ppcme2} (\ppcme) and the Penn Parsed Corpus of Modern British English \citep{ppcmbe} (\ppcmbe).   While there has been much linguistics research based on these corpora, there is relatively little previous NLP work using these corpora.  \citet{kulick-etal-2014-penn} described parsing \ppcmbe, while \citet{moon-baldridge-2007-part} and \citet{yang-eisenstein-2016-part}  focused on \pos-tagging, the former on  \ppcme, and the latter on \ppceme and \ppcmbe. 

This previous work  has discussed characteristics of these corpora that differ from that of the \ptb and the impact it might have on models trained on these corpora.   A focus has been on how to transform the annotation to be closer to that of the \ptb, such as by transforming the phrase structure \citep{kulick-etal-2014-penn} or by mapping the \ppcme \pos tag set into that of \ptb \citep{moon-baldridge-2007-part,yang-eisenstein-2016-part}.

%Regarding function tag recovery, while there has been no previous work on recovering the function tags from these corpora that we are aware of, there has been work on recovering the function tag from other corpora, in particular the \ptb, such as in \citet{blaheta-charniak-2000-assigning,blahetadiss,gabbard-etal-2006-fully,merlo-musillo-2005-accurate}.
%We follow the approach of \citet{gabbard-etal-2006-fully}, in which the function are simply not deleted for %training, and labels such as {\tt NP-SBJ} are treated as atomic units.  

%\footnote{\textbf{Stuff I've come across that maybe we  should mention: \cite{yang2017robust},  \cite{smith2019enhancing}, \cite{schneider2017comparing}, \cite{schneider2015parsing}.  Maybe something about the EarlyPrint group, especially if we might want to get in touch with them. }}


